A well balanced fvc scheme for 2d shallow water flows on unstructured triangular meshes

We consider in this work the numerical resolution of a 2D shallow water system with a Coriolis effect and bottom friction stresses on unstructured meshes by a new Finite Volume Characteristics (FVC) scheme, which has been introduced in the preliminary works that will be cited below. Our main goal is to extend this approach to 2D unstructured formalism while preserving the physical and mathematical properties of the system, including the C-property. First, we present our extension by preserving the advantages of the finite volume discretization such as conservation property and the method of characteristics such as elimination of Riemann solvers. Afterward, an approach was applied to the topography source term that leads to a well-balanced scheme satisfying the steady-state condition of still water. A semi-implicit treatment will also be presented in this study to avoid stability problems for the other source terms. Finally, the proposed finite volume method is verified on several benchmark tests and shows good agreement with analytical solutions and experimental results; moreover, it gives a noticeable accuracy and rapidity improvement compared to the original approaches.

==> Chapitres/references.tex <==
\begin{thebibliography}{10}

\bibitem{benkhaldoun2012numerical}
Fayssal Benkhaldoun, Salah Daoudi, Imad Elmahi, and Mohammed Sea{\"\i}d.
\newblock Numerical modelling of sediment transport in the nador lagoon
  (morocco).
\newblock {\em Applied Numerical Mathematics}, 62(12):1749--1766, 2012.

\bibitem{benkhaldoun2013unstructured}
Fayssal Benkhaldoun, Imad Elmahi, Saida Sari, and Mohammed Sea{\"\i}d.
\newblock An unstructured finite-volume method for coupled models of suspended
  sediment and bed load transport in shallow-water flows.
\newblock {\em International journal for numerical methods in fluids},
  72(9):967--993, 2013.

\bibitem{chaabelasri2014well}
EM~Chaabelasri, I~Elmahi, R~Abdellaoui, and N~Salhi.
\newblock Well balanced adaptive simulation of pollutant transport by shallow
  water flows: Application to the bay of tangier.
\newblock {\em International Journal of Hydraulic Engineering}, 3(1):10--23,
  2014.

\bibitem{ferrari2004new}
Stefania Ferrari and Fausto Saleri.
\newblock A new two-dimensional shallow water model including pressure effects
  and slow varying bottom topography.
\newblock {\em ESAIM: Mathematical Modelling and Numerical
  Analysis-Mod{\'e}lisation Math{\'e}matique et Analyse Num{\'e}rique},
  38(2):211--234, 2004.

\bibitem{benkhaldoun2010new}
Fayssal Benkhaldoun, Imad Elmahi, and Mohammed Sea{\"\i}d.
\newblock A new finite volume method for flux-gradient and source-term
  balancing in shallow water equations.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  199(49-52):3324--3335, 2010.

\bibitem{bermudez1998upwind}
Alfredo Berm{\'u}dez, Alain Dervieux, Jean-Antoine Desideri, and M~Elena
  V{\'a}zquez.
\newblock Upwind schemes for the two-dimensional shallow water equations with
  variable depth using unstructured meshes.
\newblock {\em Computer methods in applied mechanics and engineering},
  155(1-2):49--72, 1998.

\bibitem{bermudez1994upwind}
Alfredo Bermudez and Ma~Elena Vazquez.
\newblock Upwind methods for hyperbolic conservation laws with source terms.
\newblock {\em Computers \& Fluids}, 23(8):1049--1071, 1994.

\bibitem{leveque1998balancing}
Randall~J LeVeque.
\newblock Balancing source terms and flux gradients in high-resolution godunov
  methods: the quasi-steady wave-propagation algorithm.
\newblock {\em Journal of computational physics}, 146(1):346--365, 1998.

\bibitem{rebollo2003entropy}
Tom{\'a}s~Chac{\'o}n Rebollo, Antonio~Domi{\'n}guez Delgado, and Enrique
  D~Fern{\'a}ndez Nieto.
\newblock An entropy-correction free solver for non-homogeneous shallow water
  equations.
\newblock {\em ESAIM: Mathematical Modelling and Numerical Analysis},
  37(5):755--772, 2003.

\bibitem{rebollo2003family}
Tom{\'a}s~Chac{\'o}n Rebollo, Antonio~Dom{\i}́nguez Delgado, and Enrique
  D~Fern{\'a}ndez Nieto.
\newblock A family of stable numerical solvers for the shallow water equations
  with source terms.
\newblock {\em Computer methods in applied mechanics and engineering},
  192(1-2):203--225, 2003.

\bibitem{castro2017well}
Manuel~J Castro, Sergio Ortega, and Carlos Par{\'e}s.
\newblock Well-balanced methods for the shallow water equations in spherical
  coordinates.
\newblock {\em Computers \& Fluids}, 157:196--207, 2017.

\bibitem{michel2017well}
Victor Michel-Dansac, Christophe Berthon, St{\'e}phane Clain, and
  Fran{\c{c}}oise Foucher.
\newblock A well-balanced scheme for the shallow-water equations with
  topography or manning friction.
\newblock {\em Journal of Computational Physics}, 335:115--154, 2017.

\bibitem{vukovic2002eno}
Senka Vukovic and Luka Sopta.
\newblock Eno and weno schemes with the exact conservation property for
  one-dimensional shallow water equations.
\newblock {\em Journal of Computational Physics}, 179(2):593--621, 2002.

\bibitem{perthame2001kinetic}
Benoit Perthame and Chiara Simeoni.
\newblock A kinetic scheme for the saint-venant system with a source term.
\newblock {\em Calcolo}, 38(4):201--231, 2001.

\bibitem{benkhaldoun2010simple}
Fayssal Benkhaldoun and Mohammed Sea{\"\i}d.
\newblock A simple finite volume method for the shallow water equations.
\newblock {\em Journal of computational and applied mathematics},
  234(1):58--72, 2010.

\bibitem{benkhaldoun2015projection}
Fayssal Benkhaldoun, Saida Sari, and Mohammed Sea{\"\i}d.
\newblock Projection finite volume method for shallow water flows.
\newblock {\em Mathematics and computers in simulation}, 118:87--101, 2015.

\bibitem{benkhaldoun2015family}
Fayssal Benkhaldoun, Saida Sari, and Mohammed Sea{\"\i}d.
\newblock A family of finite volume eulerian--lagrangian methods for
  two-dimensional conservation laws.
\newblock {\em Journal of computational and applied mathematics}, 285:181--202,
  2015.

\bibitem{gerbeau2000derivation}
Jean-Fr{\'e}d{\'e}ric Gerbeau and Beno{\^\i}t Perthame.
\newblock Derivation of viscous saint-venant system for laminar shallow water;
  numerical validation.
\newblock 2000.

\bibitem{delestre2010simulation}
Olivier Delestre.
\newblock {\em Simulation du ruissellement d'eau de pluie sur des surfaces
  agricoles}.
\newblock PhD thesis, Universit{\'e} d'Orl{\'e}ans; Universit{\'e}
  d'Orl{\'e}ans, 2010.

\bibitem{hervouet2007hydrodynamics}
Jean-Michel Hervouet.
\newblock {\em Hydrodynamics of free surface flows: modelling with the finite
  element method}, volume 360.
\newblock Wiley Online Library, 2007.

\bibitem{zaouali2008structure}
Sahbi Zaouali.
\newblock {\em Structure et mod{\'e}lisation d'{\'e}coulements {\`a} surface
  libre dans des canaux de rugosit{\'e} inhomog{\`e}ne}.
\newblock PhD thesis, 2008.

\bibitem{godlewski2013numerical}
Edwige Godlewski and Pierre-Arnaud Raviart.
\newblock {\em Numerical approximation of hyperbolic systems of conservation
  laws}, volume 118.
\newblock Springer Science \& Business Media, 2013.

\bibitem{serre1999systems}
Denis Serre.
\newblock {\em Systems of Conservation Laws 1: Hyperbolicity, entropies, shock
  waves}.
\newblock Cambridge University Press, 1999.

\bibitem{olbers2012ocean}
Dirk Olbers, J{\"u}rgen Willebrand, and Carsten Eden.
\newblock {\em Ocean dynamics}.
\newblock Springer Science \& Business Media, 2012.

\bibitem{gassner2016well}
Gregor~J Gassner, Andrew~R Winters, and David~A Kopriva.
\newblock A well balanced and entropy conservative discontinuous galerkin
  spectral element method for the shallow water equations.
\newblock {\em Applied Mathematics and Computation}, 272:291--308, 2016.

\bibitem{lions1996existence}
Pierre-Louis Lions, Beno{\^\i}t Perthame, and Panagiotis~E Souganidis.
\newblock Existence and stability of entropy solutions for the hyperbolic
  systems of isentropic gas dynamics in eulerian and lagrangian coordinates.
\newblock {\em Communications on pure and applied mathematics}, 49(6):599--638,
  1996.

\bibitem{fjordholm2011well}
Ulrik~S Fjordholm, Siddhartha Mishra, and Eitan Tadmor.
\newblock Well-balanced and energy stable schemes for the shallow water
  equations with discontinuous topography.
\newblock {\em Journal of Computational Physics}, 230(14):5587--5609, 2011.

\bibitem{ziggaf2020fvc}
Moussa Ziggaf, Mohamed Boubekeur, Fayssal Benkhaldoun, Imad El~Mahi, and Imad
  Kissami.
\newblock The {FVC} scheme on unstructured meshes for the two-dimensional
  shallow water equations.
\newblock In {\em International Conference on Finite Volumes for Complex
  Applications}, pages 455--465. Springer, 2020.

\bibitem{roe1986characteristic}
Philip~L Roe.
\newblock Characteristic-based schemes for the euler equations.
\newblock {\em Annual review of fluid mechanics}, 18(1):337--365, 1986.

\bibitem{seaid2001quasi}
Mohammed Sea{\"\i}d.
\newblock On the quasi-monotone modified method of characteristics for
  transport-diffusion problems with reactive sources.
\newblock {\em Computational Methods in Applied Mathematics Comput. Methods
  Appl. Math.}, 2(2):186--210, 2001.

\bibitem{fjordholm2011vorticity}
Ulrik~S Fjordholm and Siddhartha Mishra.
\newblock Vorticity preserving finite volume schemes for the shallow water
  equations.
\newblock {\em SIAM Journal on Scientific Computing}, 33(2):588--611, 2011.

\bibitem{monthe1999positivity}
LA~Monthe, F1~Benkhaldoun, and I~Elmahi.
\newblock Positivity preserving finite volume roe: schemes for
  transport-diffusion equations.
\newblock {\em Computer Methods in Applied Mechanics and Engineering},
  178(3-4):215--232, 1999.

\bibitem{roe1981approximate}
Philip~L Roe.
\newblock Approximate riemann solvers, parameter vectors, and difference
  schemes.
\newblock {\em Journal of computational physics}, 43(2):357--372, 1981.

\bibitem{dafermos2005hyperbolic}
Constantine~M Dafermos.
\newblock {\em Hyperbolic conservation laws in continuum physics}, volume~3.
\newblock Springer, 2005.

\bibitem{stoker1948formation}
James~J Stoker.
\newblock The formation of breakers and bores the theory of nonlinear wave
  propagation in shallow water and open channels.
\newblock {\em Communications on Pure and Applied Mathematics}, 1(1):1--87,
  1948.

\bibitem{stoker2011water}
James~Johnston Stoker.
\newblock {\em Water waves: The mathematical theory with applications},
  volume~36.
\newblock John Wiley \& Sons, 2011.

\bibitem{henderson1966macmillan}
FM~Henderson.
\newblock Open channel flow. macmillan series in civil engineering.
\newblock {\em New York}, 1966.

\bibitem{fennema1989implicit}
Robert~J Fennema and M~Hanif~Chaudhry.
\newblock Implicit methods for two-dimensional unsteady free-surface flows.
\newblock {\em Journal of hydraulic research}, 27(3):321--332, 1989.

\bibitem{audusse2000kinetic}
Emmanuel Audusse, Marie-Odile Bristeau, and Benoit Perthame.
\newblock {\em Kinetic schemes for Saint-Venant equations with source terms on
  unstructured grids}.
\newblock PhD thesis, INRIA, 2000.

\bibitem{fennema1990explicit}
Robert~J Fennema and M~Hanif Chaudhry.
\newblock Explicit methods for 2-d transient free surface flows.
\newblock {\em Journal of Hydraulic Engineering}, 116(8):1013--1034, 1990.

\bibitem{zhou2001surface}
Jian~G Zhou, Derek~M Causon, Clive~G Mingham, and David~M Ingram.
\newblock The surface gradient method for the treatment of source terms in the
  shallow-water equations.
\newblock {\em Journal of Computational physics}, 168(1):1--25, 2001.

\bibitem{wang2020new}
Zhenming Wang, Jun Zhu, and Ning Zhao.
\newblock A new fifth-order finite difference well-balanced multi-resolution
  weno scheme for solving shallow water equations.
\newblock {\em Computers \& Mathematics with Applications}, 80(5):1387--1404,
  2020.

\bibitem{kuo2000nonlinear}
Allen~C Kuo and Lorenzo~M Polvani.
\newblock Nonlinear geostrophic adjustment, cyclone/anticyclone asymmetry, and
  potential vorticity rearrangement.
\newblock {\em Physics of Fluids}, 12(5):1087--1100, 2000.

\bibitem{frazao2002dam}
S~Soares Fraz{\~a}o and Y~Zech.
\newblock Dam break in channels with 90 bend.
\newblock {\em Journal of Hydraulic Engineering}, 128(11):956--968, 2002.

\bibitem{guan2013robust}
M~Guan, NG~Wright, and PA~Sleigh.
\newblock A robust 2d shallow water model for solving flow over complex
  topography using homogenous flux method.
\newblock {\em International Journal for Numerical Methods in Fluids},
  73(3):225--249, 2013.

\bibitem{zhou2002numerical}
Jian~G Zhou, Derek~M Causon, David~M Ingram, and Clive~G Mingham.
\newblock Numerical solutions of the shallow water equations with discontinuous
  bed topography.
\newblock {\em International journal for numerical methods in fluids},
  38(8):769--788, 2002.

\bibitem{audusse2014fast}
Emmanuel Audusse, Fayssal Benkhaldoun, Saida Sari, Mohammed Sea{\"\i}d, and
  Pablo Tassi.
\newblock A fast finite volume solver for multi-layered shallow water flows
  with mass exchange.
\newblock {\em Journal of Computational Physics}, 272:23--45, 2014.

\bibitem{al2019new}
Alia Al-Ghosoun, Michael Herty, and Mohammed Sea{\"\i}d.
\newblock A new numerical treatment of moving wet/dry fronts in dam-break
  flows.
\newblock {\em Journal of Applied Mathematics and Computing}, 59(1):489--516,
  2019.

\bibitem{phongthanapanich2019comparative}
Sutthisak Phongthanapanich and Robert Eymard.
\newblock A comparative study of characteristic finite element and
  characteristic finite volume methods for convection-diffusion-reaction
  problems on triangular grids.
\newblock {\em Applied Science and Engineering Progress}, 12(4):235--242, 2019.

\bibitem{brennen2005fundamentals}
Christopher~Earls Brennen and Christopher~E Brennen.
\newblock Fundamentals of multiphase flow.
\newblock 2005.

\bibitem{qamar2006application}
Shamsul Qamar and Gerald Warnecke.
\newblock Application of space--time ce/se method to shallow water
  magnetohydrodynamic equations.
\newblock {\em Journal of computational and applied mathematics},
  196(1):132--149, 2006.

\bibitem{zia2014numerical}
Saqib Zia, Munshoor Ahmed, and Shamsul Qamar.
\newblock Numerical solution of shallow water magnetohydrodynamic equations
  with non-flat bottom topography.
\newblock {\em International Journal of Computational Fluid Dynamics},
  28(1-2):56--75, 2014.

\end{thebibliography}
